Convergence of Alternating Least Squares Optimisation for Rank-One Approximation to High Order Tensors

The approximation of tensors has important applications in various disciplines, but it remains an extremely challenging task. It is well known that tensors of higher order can fail to have best low-rank approximations, but with an important exception that best rank-one approximations always exists. The most popular approach to low-rank approximation is the alternating least squares (ALS) method. The convergence of the alternating least squares algorithm for the rank-one approximation problem is analysed in this paper. In our analysis we are focusing on the global convergence and the rate of convergence of the ALS algorithm. It is shown that the ALS method can converge sublinearly, Q-linearly, and even Q-superlinearly. Our theoretical results are illustrated on explicit examples.

==> MATHS/PRE_MATH.TEX <==
%%%%% Begin  LaTeX  File PRE_MATH.tex             5. Feb. 96  %%%%%%%%%%%%%%%%%
%%%%%
%%%%% Definieren mathematischer Zusatzzeichen   und Symbole
%%%%%
%%%%%            based on HEADMATH.tex      Edgar Katzer, Hamburg, Sept. 1995.
%%%%%
%%%%%            and      AMMACROS.tex     (angewandte Mathematik Hamburg) 10. 11. 89
%%%%%                     PRE_VOSS.tex      H. VOSS, Sven Loges (9/89, 10/89) Mathematik TU-Harburg
%%%%%
%%%%% Author:    Edgar Katzer, Hamburg
%%%%% Version:   Version of 11. Dec, 1995,
%%%%%
%
%
%%%%%%%%%%%%%%%%%  Spezielle mathematische Zeichen       %%%%%%
%
%
%%  Mengensymbole
%
    \newcommand    {\BbbC}  {\mbox{\rm $\scriptscriptstyle    %%  complex C
                                   ^\mid$\hspace{-0.40em}C}}
    \newcommand    {\BbbN}  {\mbox{                           %%  integer N
                            \rm I\hspace{-0.22em}I\hspace{-0.32em}N}}
    \newcommand    {\BbbK}  {\mbox{                           %%  integer N
                            \rm I\hspace{-0.22em}I\hspace{-0.32em}K}}
    \newcommand    {\BbbQ}  {\mbox{\rm $\scriptscriptstyle    %%  rational Q
                                   ^\mid$\hspace{-0.40em}Q}}
    \newcommand    {\BbbR}  {\mbox{\rm I\hspace{-0.22em}R}}   %%  real    IR
    \newcommand    {\BbbE}  {\mbox{\rm I\hspace{-0.22em}E}}   %%  euclidian IE
    \newcommand    {\BbbZ}  {\mbox{\sf Z\hspace{-0.44em}Z}}   %%  integer Z

    \newcommand    {\icom}  {\BbbC}                           %%  complex C
    \newcommand    {\inat}  {\BbbN}                           %%  integer N
    \newcommand    {\irat}  {\BbbQ}                           %%  rational Q
    \newcommand    {\iree}  {\BbbR}                           %%  real    IR
    \newcommand    {\znat}  {\BbbZ}                           %%  integer Z

    \newcommand    {\nin}   {\in \hspace{-0.80em} /}       %%  not in
%
%   from  AMMACROS.tex   10.11.89
%
 %  \def            \R      {\mbox{\makebox[.2em][l]{I}R}}
 %  \def            \B      {\mbox{\makebox[.2em][l]{I}B}}
 %  \def            \N      {\mbox{\makebox[.2em][l]{I}N}}
 %  \def            \Z      {\mbox{\makebox[.22em][l]{\sf Z}{\sf Z}}}
               %\def\Z{\mbox{\makebox[.283em][l]{Z}Z}}
 %  \def            \C      {\makebox[.6em]{\makebox[-.18em]{C}\rule{.03em}{1.5ex}}}
               %\def\C{\makebox[.8em][l]{\makebox[.25em][l]{C}\rule{.03em}{1.5ex}}}
 %  \def            \Q      {\makebox[.6em]{\makebox[-.25em]{Q}\rule{.03em}{1.5ex}}}
               %\def\Q      {\makebox[.8em][l]{\makebox[.25em][l]{Q}\rule{.03em}{1.5ex}}}
    \def            \L      {\mbox{\makebox[.2em][l]{I}L}}
    \def            \P      {\mbox{\makebox[.2em][l]{I}P}}
%
%%  Spezielle Schriftarten  ( FETT,  \sf   etc
%
    \newcommand    {\ZZ}    { \mbox{\rm\bf{Z}} }
    \newcommand    {\HH}    { {^{\mbox{\scriptsize \sf H }}} }
    \newcommand    {\TT}    { {^{\mbox{\scriptsize \sf T }}} }
%
%
%%%%%%%%%%%%%%%%%  mathematische Begriffe                 %%%%%
%
    \newcommand    {\Bild}  { \mbox{\rm Bild$\,$} }
    \newcommand    {\Kern}  { \mbox{\rm Kernel$\,$} }
    \newcommand    {\Range} { \mbox{\rm Range$\,$} }
    \newcommand    {\Diag}  { \mbox{\rm diag$\,$} }
    \newcommand    {\cond}  { \mbox{\rm cond} }
    \newcommand    {\Span}  { \mbox{\rm Span$\,$} }

    \newcommand    {\Ccone} { \mbox{\rm CCone$\,$} }
    \newcommand    {\cone}  { \mbox{\rm cone$\,$} }
    \newcommand    {\grad}  { \mbox{\rm grad$\,$} }
    \newcommand    {\even}  { \mbox{\rm even$\,$} }
    \newcommand    {\odd}   { \mbox{\rm odd$\,$} }
    \newcommand    {\sonst} { \mbox{\rm sonst$\,$} }
%
%
%%%%%%%%%%%%%%%%%  Spezielle aufwendigere neue Zeichen   %%%%%%
%
%
    \newcommand    {\C}     { \langle }
    \newcommand    {\Z}     { \rangle }

    \newcommand    {\Doe}   { \mbox{
                                \makebox[.2em][c]{$\circ$}---\makebox[.2em][c]
                                                 {$\bullet$}  }}
    \newcommand    {\doe}   { \mbox{
                                \makebox[.2em][c]{$\bullet$}---\makebox[.2em][c]
                                                 {$\circ$}   }}
%
    \newcommand    {\isotone}  {\unitlength1pt
                                    \begin{picture}(28,15)
                                        \put(8,1){  \vector(2,1){12}  }
                                    \end{picture}   }
%
    \newcommand    {\kreuz}[2] {\mbox{ \raisebox{-1.2ex}
                                  {$\stackrel {\stackrel{#2}
                                     { \displaystyle \times}  }
                                  {\scriptscriptstyle {#1}}$}}}
%
    \newcommand    { \lgo }[2] {\begin{array}[t]{c}
                                   \longrightarrow \\ {\raisebox{2ex}[-2ex]
                                      {$\scriptstyle #1 \to #2 $} }
                                \end{array} }
%
    \newcommand    {\tmid}[1]  {\raisebox{1.95ex}[-1.95ex] {#1} }
%
%%%%%
%%%%%
%%%%% End    LaTeX  File PRE_MATH.tex            11. Dec. 95  %%%%%%%%%%%%%%%%%
